OmniGlue: Generalizable Feature Matching with Foundation Model Guidance

The image matching field has been witnessing a continuous emergence of novel learnable feature matching techniques, with ever-improving performance on conventional benchmarks. However, our investigation shows that despite these gains, their potential for real-world applications is restricted by their limited generalization capabilities to novel image domains. In this paper, we introduce OmniGlue, the first learnable image matcher that is designed with generalization as a core principle. OmniGlue leverages broad knowledge from a vision foundation model to guide the feature matching process, boosting generalization to domains not seen at training time. Additionally, we propose a novel keypoint position-guided attention mechanism which disentangles spatial and appearance information, leading to enhanced matching descriptors. We perform comprehensive experiments on a suite of $7$ datasets with varied image domains, including scene-level, object-centric and aerial images. OmniGlue's novel components lead to relative gains on unseen domains of $20.9\%$ with respect to a directly comparable reference model, while also outperforming the recent LightGlue method by $9.5\%$ relatively.Code and model can be found at https://hwjiang1510.github.io/OmniGlue

==> section/04_method.tex <==
\section{Method}

% Real applications usually require the image matching model to \textit{generalize} to novel customized domains. One solution to improve the generalization capability is collecting a large-scale dataset from diverse domains for training a comprehensive model. However, due to the difficulty of getting fine-grained correspondence annotation, existing data for training image matching methods is limited. Then a question arises: How to improve the generalization capability under the restriction of using currently available training data?

We first introduce the problem formulation and our base model SuperGlue in Sec.~\ref{sec: preliminaries}, and \modelname{} is introduced in Sec.~\ref{sec: omniglue}.

% In this paper, we propose \modelname{}. We examine the prior image matching methods and build \modelname{} based on the sparse matching, i.e., SuperGlue, which employs the task-agnostic local feature descriptors. At its core, \modelname{} proposes a novel attention module to disentangle the local feature descriptors and the positional features to achieve better generalization. We also guide the inter-image keypoint information aggregation attention with a image foundation model, which provides coarse but generalizable matching cues. We introduce the details of the task definition and \modelname{} model architecture in the following sections.

\subsection{Preliminaries}
\label{sec: preliminaries}
\paragraph{Problem formulation.}
Given two images $I_A$ and $I_B$, as well as their keypoint sets $\mathbf{A} := \{A_1, ..., A_N \}$ and $\mathbf{B} := \{ B_1, ..., B_M\}$, we find the correspondence between the keypoints across image. Note that $N$ and $M$ are the number of identified keypoints of $I_A$ and $I_B$, respectively. The keypoints are identified by an off-the-shelf keypoint detector, i.e. SuperPoint~\cite{detone2018superpoint}, where each keypoint has two features: i) Local visual descriptors, and ii) Positional features. To get the keypoint positional features, we apply the positional embedding function~\cite{detone2018superpoint} on the normalized keypoint location, and we further refine it using an MLP. We denote the local descriptor and positional features of all keypoints in set $\mathbf{A}$ as $\mathbf{d}^{A} \in \mathbb{R}^{N\times C}$ and $\mathbf{p}^{A} \in \mathbb{R}^{N\times C}$, respectively. The two features of all keypoint in set $\mathbf{B}$ are denoted as $\mathbf{b}^B \in \mathbb{R}^{M\times C}$ and $\mathbf{p}^B \in \mathbb{R}^{M\times C}$.

We find the correspondence by solving the partial assignment between the keypoint sets. The output is the partial assignment matrix $\mathbf{T} \in [0,1]^{N\times M}$, where the element $\mathbf{T}_{i,j}$ represents the probability of assigning correspondence for keypoint $A_i$ and $B_j$.

\paragraph{Attention.} The Attention module~\cite{Vaswani2017Attention} is a trainable feature aggregation function, which can be formulated as:
\begin{align}
    &\text{Attention}(\mathbf{q}, \mathbf{x}) =
    \text{Softmax}(\frac{\mathbf{q}\cdot (\mathbf{x}\mathbf{W}_k)^T}{\sqrt{C}})\cdot (\mathbf{x}\mathbf{W}_v),
\end{align}
where $\mathbf{q}$ is the query tokens, $\mathbf{x}$ is the original key/value tokens, $\mathbf{W}_k$ and $\mathbf{W}_v$ are weights to map $\mathbf{x}$ into key and value tokens -- they are from the same source $\mathbf{x}$. The normalized feature similarities between the query and key tokens serve as the aggregation weights. We omit the mapping weights applied on query tokens and the multiple heads in the attention for clarity.

\paragraph{SuperGlue Contextual Reasoning.}
SuperGlue uses Graph Neural Network (GNN) to propagate information between keypoints, leveraging the correlation between keypoints as the contextual information to refine keypoint representations. Specifically, the GNN is modeled as attention layers, where each keypoint is densely connect to all other keypoints.
The information propagation process is performed in an iterative manner, composed of intra-image and inter-image keypoint information passing. Taking refinement process of keypoints sets $\mathbf{A}$ of image $I^A$ as an example, it is formulated as:
\begin{align}
\mathbf{f}^{A} \leftarrow \mathbf{f}^A + \text{MLP}([\mathbf{f}^A \vert \Delta\mathbf{f}^A]),\\
\Delta\mathbf{f}^A = \text{Attention}(\text{q}= \mathbf{f}^A, \text{x}=\cdot)
\end{align}
where $\mathbf{f}$ denotes the keypoint representation, $\leftarrow$ denotes the updating of features, and $[\cdot\vert \cdot]$ is the concatenation operation. For intra-image keypoint information passing, the key/value token is the keypoint representation itself ($\mathbf{x}=\mathbf{f}^{A}$, as a self-attention block); For inter-image keypoint information passing, the key/value token is the representation of keypoints in the other image ($\mathbf{x}=\mathbf{f}^{B}$, as a cross-attention block).

In detail, the keypoint representation entangles both keypoint local descriptors and positional features as 
\begin{align}
\label{eq: sg_kp_rep}
    \mathbf{f} = \mathbf{d} + \mathbf{p}.
\end{align}
The SuperGlue keypoint representation $\mathbf{f}$ is initialized before the first attention layer. Intuitively, the information passing process considers both visual and spatial cues. We observe that the entangled representation limits the generalization capability of SuperGlue - it is overly dependent on positional cues for information passing, which is vulnerable under images captured by out-of-distribution relative camera poses.


\begin{figure*}[t]

    \begin{center}
    \includegraphics[width=0.7\linewidth]{images/TODO - block diagram.png}
    \end{center}
    
    \caption{
    \colorbox{yellow}{\textbf{TODO: Architecture diagram of our method.}} Consider using DINO visualizations to show the similarity of DINO features across semantically similar parts.
    }
    
    \label{fig:method}
\end{figure*}

\subsection{\modelname{} Architecture}
\label{sec: omniglue}
\paragraph{Overview.} As shown in Fig.~\ref{}, following SuperGlue, we leverage attention layers to perform contextual reasoning and refine the representation of keypoints. Different from SuperGlue, which entangles keypoint positional features and local descriptors during the process (described in Eq.~\ref{eq: sg_kp_rep}), we disentangle them when performing contextual reasoning. In detail, we leverage both positional features and local descriptors to correlate keypoints, enabling the model to learn position-related matching priors. The update of keypoint representation, however, is only composed by local descriptors. This disentanglement prevents the matching from being overly reliant on the keypoint positions information, enabling \modelname{} to generalize to new domain with different camera pose transformations.

Furthermore, we leverage an image foundation model DINO~\cite{Oquab2023DINOv2}, which is trained on large-scale data from diverse domains, to improve the generalization capability of \modelname{}. Prior works have demonstrated the robust semantic correspondence properties of the image foundation models~\cite{Zhang2023ATO}. However, the granularity of the correspondences yielded from the DINO image features is limited. Instead of directly using DINO image features for matching keypoints, we choose to leverage DINO to guide the inter-image information propagation process.

For any query keypoint, we identify the potential matching set, which is the keypoints in the other image with high DINO feature similarities. Due to the robustness of DINO, the ground-truth matching keypoint would be included in the potential matching set with high possibility even in a novel domain. We only propagate information from the potential matching set, instead of all keypoints in the other image, to the query keypoint. Theoretically, it prunes the densely-connected graph between keypoints of two images.
With the guidance of DINO similarities, information from irrelevant keypoints will be rejected from being fused into the query keypoint features. Moreover, it encourages the attention modules to focus on distinguishing the ground-truth matching point in the smaller potential matching set. Note that we do not forcibly limit the matching candidate space as the potential matching set, as the DINO may also be incorrect in some cases. DINO guidance is only considered during inter-image information propagation process.

We introduce the details of our proposed techniques in the following section.


\paragraph{Keypoint Feature Representation.} We represent the keypoint only with their local descriptors $\mathbf{d}$ -- their positional features $\mathbf{p}$ should not be incorporated to compute the similarity matrix $\mathbf{S} = \mathbf{d}^{A} \cdot (\mathbf{{d}}^{B})^{T}$. The reason is that keypoints from the two images with similar locations are not necessary to be matched. However, the positional feature components of the SuperGlue keypoint representation lead to higher similarity scores for keypoints with similar locations.


\paragraph{Disentangle Positional Features.} As positional features provide cues to understand spatial correlation between keypoints and is useful for learning rigid priors, we incorporate them in contextual reasoning. It is enabled by an attention module where the \textit{key and value are from different sources}. This attention module can be formulated as 
\begin{align}
    \text{Attention}(\mathbf{q}, \mathbf{k}, \mathbf{v}) = \text{Softmax}(\frac{\mathbf{q}\mathbf{k}^T}{\sqrt{C}})\cdot \mathbf{v},\quad  \mathbf{k}\neq \mathbf{v},
\end{align}
where $c$ is the channel size of inputs.


\paragraph{Intra-image Self-Attention.} This block performs information propagation between keypoints from the same image, where each keypoint attends from all keypoints. The inputs are local descriptors and positional features of the keypoints, and the output is the updated local descriptors. We take the example of refining keypoint descriptors of image $I_A$. With the attention module defined above, we formulate the intra-image information passing of keypoint set $\mathbf{A}$ as 
\begin{align}
\mathbf{d}^A \leftarrow \mathbf{d}^A + \text{MLP}([\mathbf{d}^A \vert \Delta \mathbf{d}^A_{slf}]), \text{where}\\
\Delta \mathbf{d}^A_{slf} = \text{Attention}(\mathbf{q}^A, \mathbf{k}^A, \mathbf{v}^A), \text{and}\\
\mathbf{q}^A = \text{MLP}^q_{slf}(\mathbf{d}^A + \mathbf{p}^A), \\
\mathbf{k}^A = \text{MLP}^k_{slf}(\mathbf{d}^A + \mathbf{p}^A), \\
\mathbf{v}^A = \text{MLP}^v_{slf}(\mathbf{d}^A).
\end{align}
In detail, the query $\mathbf{q}^A$ and the key $\mathbf{k}^A$ of the attention are composed of both keypoint local descriptors and positional features. We fuse the information with an MLP layer. In contrast, the value $\mathbf{v}^A$ is only composed of local descriptors. Intuitively, the query and key compute the attention weights, where both feature affinity and spatial correlations are considered. The final output of the attention, denoted as $\Delta\mathbf{d}^A$, is the weighted value tokens, which is only composed of local descriptor components. We note that the descriptors are updated through the contextual reasoning layers and the positional features are fixed. The MLP$^q_{slf}$, MLP$^k_{slf}$ and MLP$^v_{slf}$ are not shared across different attention modules.


\paragraph{Inter-image Cross-Attention.} This block performs information propagation between keypoints from different images, e.g. using information of keypoint set $\mathbf{B}$ to update the features of set $\mathbf{A}$. In detail, each keypoint $A_i$ of set $\mathbf{A}$ attends to its potential matching set, which is a subset of $\mathbf{B}$. 

To identify the potential matching set, we leverage the image foundation model DINO. We extract features of the images $I_A$ and $I_B$, and interpolate them at the keypoint locations. We denote the DINO features of the two keypoint sets as $\mathbf{g}^A \in \mathbb{R}^{N\times C'}$ and $\mathbf{g}^B \in \mathbb{R}^{M\times C'}$. We compute the pairwise similarity matrix $\mathbf{G} = \mathbf{g}^A \cdot (\mathbf{g}^B)^T \in \mathbb{R}^{N\times M}$. The $i^{th}$ row of the matrix $\mathbf{G}$, denoted as $\mathbf{G}_i \in \mathbb{R}^{M}$, represents the DINO feature similarity between keypoint $A_i$ and all keypoints in set $\mathbf{B}$. We select $K$ keypoints with highest DINO similarity as the potential matching set. The result forms a mask $\mathbf{M} \in \mathbb{R}^{N\times M}$, where the elements that correspond to the potential matching set are set to $1$ (positive).

The cross-attention between keypoints and their potential matching set can be formulated as:
\begin{align}
    \mathbf{d}^A \leftarrow \mathbf{d}^A + \text{MLP}([\mathbf{d}^A \vert \Delta \mathbf{d}^A_{crs}]), \text{where}\\
    \Delta \mathbf{d}^A_{crs} = \text{MaskedAttention}(\mathbf{q}^A, \mathbf{k}^B, \mathbf{v}^B \vert \mathbf{M}), \text{and}\\
    \mathbf{q}^A = \text{MLP}^q_{crs}(\mathbf{d}^A + \mathbf{p}^A), \\
    \mathbf{k}^B = \text{MLP}^k_{crs}(\mathbf{d}^B + \mathbf{p}^B), \\
    \mathbf{v}^B = \text{MLP}^v_{crs}(\mathbf{d}^B).
\end{align}
Within the masked attention module, the attention weights of the positive elements (potential matching set) are summed up as $1$. The attention weights of keypoints that are not in the potential matching set are $0$ (not attended). The details of the masked attention module is included in the supplementary.

We note that the keypoint set $\mathbf{B}$ is updated in a similar way with intra- and inter-image information propagation.

\paragraph{Matching Layer.} With the keypoint sets with their updated descriptors $\bar{\mathbf{d}}^A$ and $\bar{\mathbf{d}}^B$, the final correspondence results is predicted with a matching layer. Following SuperGlue~\cite{sarlin2020superglue}, we first compute the similarity matrix $\mathbf{S} = \bar{\mathbf{d}}^A \cdot (\bar{\mathbf{d}}^B)^{T}$. Then the partial assignment matrix $\mathbf{T}$ is predicted as the optimal transportation using the Sinkhorn algorithm.






